B-HAR: an open-source baseline framework for in depth study of human activity recognition datasets and workflows

Human Activity Recognition (HAR), based on machine and deep learning algorithms is considered one of the most promising technologies to monitor professional and daily life activities for different categories of people (e.g., athletes, elderly, kids, employers) in order to provide a variety of services related, for example to well-being, empowering of technical performances, prevention of risky situation, and educational purposes. However, the analysis of the effectiveness and the efficiency of HAR methodologies suffers from the lack of a standard workflow, which might represent the baseline for the estimation of the quality of the developed pattern recognition models. This makes the comparison among different approaches a challenging task. In addition, researchers can make mistakes that, when not detected, definitely affect the achieved results. To mitigate such issues, this paper proposes an open-source automatic and highly configurable framework, named B-HAR, for the definition, standardization, and development of a baseline framework in order to evaluate and compare HAR methodologies. It implements the most popular data processing methods for data preparation and the most commonly used machine and deep learning pattern recognition models.

==> algo/algo.tex <==
\begin{algorithm} % enter the algorithm environment
\caption{Structures} % give the algorithm a caption
\label{alg1} % and a label for \ref{} commands later in the document
\begin{algorithmic} % enter the algorithmic environment
    \STATE $e\textsubscript{i} = \{$
    \STATE \hskip \algorithmicindent $src\_node$,
    \STATE \hskip \algorithmicindent $dst\_node$,
    \STATE \hskip \algorithmicindent $direction$,
    \STATE \hskip \algorithmicindent $distance$
    \STATE \}
\end{algorithmic}
\end{algorithm}


\begin{algorithm} % enter the algorithm environment
\caption{Graph initialization} % give the algorithm a caption
\label{alg1} % and a label for \ref{} commands later in the document
\begin{algorithmic} % enter the algorithmic environment
    \REQUIRE $D = \{ e\textsubscript{1}, e\textsubscript{2}, e\textsubscript{n} \}, G = \{\} $
    \FORALL {$e$ in $D$}
        \IF {$e.src\_node$ !in $G$}
            \STATE $G$.append($e.src\_node$)
        \ENDIF
        %\STATE        
        \IF {$e.dst\_node$ !in $G$}
            \STATE $G$.append($e.dst\_node$)
        \ENDIF
        %\STATE
        \STATE $G[e.src\_node].edges$.append($e.direction$, \{
                \STATE \hskip \algorithmicindent dst\_node: $e.dst\_node$,
                \STATE \hskip \algorithmicindent distance: $e.distance$
        \STATE\})
    \ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm} % enter the algorithm environment
\caption{Add node} % give the algorithm a caption
\label{alg1} % and a label for \ref{} commands later in the document
\begin{algorithmic} % enter the algorithmic environment
    \REQUIRE $node, parent\_node, direction, distance, D = \{ e\textsubscript{1}, e\textsubscript{2}, e\textsubscript{n} \}, G = \{\} $
    \STATE $G$.append($node$)
    \IF{$parent\_node.edges[direction]$ exists}
        \STATE $G[node].edges$.append($direction$, \{
            \STATE \hskip \algorithmicindent dst\_node: $parent\_node.edges[direction].dst\_node$,
            \STATE \hskip \algorithmicindent distance: $parent\_node.edges[direction].distance$
        \STATE \})
        %\STATE
        \STATE $G[parent\_node].edges[direction]$ = \{
            \STATE \hskip \algorithmicindent dst\_node: $node$,
            \STATE \hskip \algorithmicindent distance: $distance$
        \STATE \}
        %\STATE
        \STATE $G[node].edges$.append($direction^{-1}$, \{
            \STATE \hskip \algorithmicindent dst\_node: $parent\_node$,
            \STATE \hskip \algorithmicindent distance: $distance$
        \STATE \})
        %\STATE
        \STATE $dst\_node$ = $node.edges[direction].dst\_node$
        \STATE $G[dst\_node].edges[direction^{-1}]$ = \{
            \STATE \hskip \algorithmicindent dst\_node: $node$,
            \STATE \hskip \algorithmicindent distance: $node.edges[direction].distance$
        \STATE \})
    \ELSE
        \STATE $G[parent\_node].edges$.append($direction$, \{
            \STATE \hskip \algorithmicindent dst\_node: $node$,
            \STATE \hskip \algorithmicindent distance: $distance$
        \STATE \})
        %\STATE
        \STATE $G[node].edges$.append($direction^{-1}$, \{
            \STATE \hskip \algorithmicindent dst\_node: $parent\_node$,
            \STATE \hskip \algorithmicindent distance: $distance$
        \STATE \})
    \ENDIF
\end{algorithmic}
\end{algorithm}

==> sec/back.tex <==
% !TEX root = ../main.tex
\section{Preliminaries}\label{sec:back}
\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\textwidth,page={3}]{imm/p_figures.pdf}
\caption{Overview of the B-HAR structure.}\label{fig:b-har_structure}
\end{figure*}
%\canc{Nowadays, sensors are becoming a prevalent presence in daily life~\cite{demrozi2020human,rault2017survey} mainly since they are integrated into our electronic devices (e.g., smartphones, smartwatches, video cameras, or smart thermostats).
%Such devices, and the integrated sensors, perceive and collect most of the data on which HAR models rely since they directly measure human movements. 
%In particular, accelerometers, gyroscopes, or heart rate sensors provide direct knowledge of body acceleration, angular velocity, and heartbeats. 
%Such information is cardinal in recognizing activities such as walking, running, standing, doing stairs, and even related to the emotional state as agitation, stress, etc. 
%However, the perceived data are noisy and not easily interpretable, requiring to be processed through particular techniques that enhance the structural characteristics.}
This section offers an overview of basic pattern recognition techniques exploiting machine and deep learning, and data preprocessing techniques (e.g., noise removal, data balancing, segmentation or feature extraction), which have been considered in B-HAR.
%, and wearable/environmental sensors market evolution.

%--------------------------------------------------------------------------
\subsection{Machine learning overview}
Classical Machine Learning (CML) algorithms are categorized into two major groups: unsupervised learning (aka clustering) and supervised learning. 
Unsupervised learning aims to identify existing patterns in input data without any information regarding the output~\cite{bishop2006pattern}. %~\cite{liu2016action}. 
Instead, supervised learning aims to construct a mathematical model that exemplifies the relationship between input and output training data. 
Besides, one or more preprocessing steps can be necessary, including feature extraction, segmentation, normalization, signal noise removal, data balancing, or features projection~\cite{domingos2012few}. 
The resulting model is applied to predict the outcome of unseen data samples. 
The most common CML algorithms are Naïve Bayes (NB), k-means clustering, Support Vector Machine (SVM), Random Forests (RF), Decision Trees (DT), and k-Nearest Neighbours (k-NN). 

\add{However,} in the last decade, Deep Learning (DL) algorithms have become popular in many domains \add{imposing itself as the new state-of-the-art HAR standard}. %~\cite{liu2016action}. 
Starting from raw input data, DL techniques automatically identify optimal features that otherwise would remain unknown without any human knowledge~\cite{shickel2017deep}. 
Nevertheless, DL models present some limitation~\cite{marcus2018deep}: data interpretation is not easy (black box model) and DL requires large datasets  and high computational devices for training.
The most common DL models are: Convolutional Neural Network (CNN), Recurrent Neural Networks (RNNs), and Long Short-Term Memory Networks (LSTMs)%, Gated Recurrent Unit (GRU), Stacked Autoencoders, Temporal Convolutional Network (TCN), and VAriational Autoencoders (VAE)
~\cite{brownlee2016master}.

%--------------------------------------------------------------------------
\subsection{Data preprocessing}
Besides the pattern recognition models, an essential step in HAR workflow is the preprocessing of raw data. 
This is necessary since raw data perceived by sensors are generally affected by different issues~\cite{shoaib2015survey} as hardware and environmental noise, errors related to null and/or missing values, and user errors made during the collection phase. 
In addition, the data can present unbalanced distribution of classes (unbalanced datasets) or require the extraction of specific features before being elaborated.
The data preprocessing step aims to reduce the effect of such issues and prepare the data for the model training phase~\cite{joshi2017artificial}. 

Concerning the hardware noise, in the literature, most of the existing techniques make use of digital filters as lowpass, highpass, bandpass, or statistical filters~\cite{nardi2019human,ordonez2016deep,li2019applying} as the Kalman %,hassan2018robust
filter~\cite{zhu2019human}. 
Furthermore, the unbalanced datasets issue is usually handled, through specific techniques, by reducing/increasing the number of samples in the most/less populated class~\cite{imbalance}. 
Finally, since raw data does not provide interpretable characteristics, feature extraction approaches are adopted to derive interpretable characteristics in the time and frequency domains. 
However, no existing standard shows the correct order in which the previous preprocessing steps should be applied. 
%Furthermore, they are directly dependent on the input data, making a preliminary study of the input signals is necessary.
